PULSE: Accelerating Distributed Pointer-Traversals on Disaggregated Memory (Extended Version)

Caches at CPU nodes in disaggregated memory architectures amortize the high data access latency over the network. However, such caches are fundamentally unable to improve performance for workloads requiring pointer traversals across linked data structures. We argue for accelerating these pointer traversals closer to disaggregated memory in a manner that preserves expressiveness for supporting various linked structures, ensures energy efficiency and performance, and supports distributed execution. We design PULSE, a distributed pointer-traversal framework for rack-scale disaggregated memory to meet all the above requirements. Our evaluation of PULSE shows that it enables low-latency, high-throughput, and energy-efficient execution for a wide range of pointer traversal workloads on disaggregated memory that fare poorly with caching alone.

==> format/margins.tex <==
\setlength{\parskip}{0pt}
\setlength{\textfloatsep}{ 4pt plus 1.0pt minus 2.0pt} % 20.0pt plus 2.0pt minus 4.0pt
\setlength{\floatsep}    { 4pt plus 1.0pt minus 2.0pt} % 12.0pt plus 2.0pt minus 2.0pt
\setlength{\intextsep}   { 4pt plus 1.0pt minus 2.0pt} % 12.0pt plus 2.0pt minus 2.0pt


==> tex/discussion.tex <==
% !TEX root = ../paper.tex
\section{Limitations \& Future Research}
\label{sec:discussion}

We discuss the limitations of our approach along with potential future research that could address them.

\paragraphb{Enabling near-memory synchronization} Since \name accelerators host multiple cores and pipelines, concurrent pointer traversals require synchronization. Our current design assumes that such synchronization is managed by the application by acquiring locks before sending requests to the offload engine, and releasing them once the requests are complete. However, synchronizing requests at the compute node can degrade the utilization of \name accelerators, since they cannot process concurrent requests on the same data while the original request is in flight. It is possible to resolve this with support for atomic memory instructions and/or synchronization APIs as a part of \name ISA; we leave the exploration of such primitives to future work.

% compute <-> memory
\paragraphb{Cache coherent pointer traversals} If data resident in a compute blade's cache is accessed on disaggregated memory via \name accelerators, it can result in consistency issues --- especially if the cached data is dirty. \name relies on application-level synchronization to protect the shared data, \ie, applications must write dirty cached data back to the memory node before submitting a new pointer-traversal request may access such data. A potentially more efficient solution could be to provide coherence between compute and memory nodes, similar to recent work on disaggregated database systems~\cite{zhang2022_teleport}.

% richer ISA
\paragraphb{Leveraging data-centric parallelism} While \name supports essential arithmetic operations by supporting arbitrary computing operations, some data-centric operations (\S\ref{ssec:compute_node}), such as vectorized operations, can be accelerated by supporting special instructions --- \eg, single instruction multiple data (SIMD) instructions such as AVX in x86. Since such an extension would increase the complexity of the logic pipeline in \name accelerator --- and consequently, energy consumption --- careful investigation will be required to realize them.

% limitation in the scratchpad
\paragraphb{Supporting arbitrary size of \code{scratch\_pad}} Data structures with complex pointer traversal logic may require more temporary space than \name's fixed-sized \code{scratch\_pad}. For instance, traversing a graph with millions of edges and vertices may require a stack- or queue-like local data structure to record if an edge or a vertex has been visited. However, increasing the size of \code{scratch\_pad} would be eventually limited by the maximum number of registers that can be physically realized in the workspace (\S\ref{ssec:acc_design}). One potential solution would be to introduce a swap space for \code{scratch\_pad} on the SmartNIC DRAM, similar to the memory hierarchy in the traditional CPU architectures. Such a design would require careful consideration since it would break \name's assumption of deterministic computation time ($t_c$) and make enforcement based on $\eta$ more involved (\S\ref{ssec:compute_node}). It may be possible to exploit algorithmic upper bounds of stacks and queues to guarantee deterministic execution ($t_c$) --- we leave their exploration to future work. 
% perf isol.
\paragraphb{Fairness and isolation for multi-tenancy} A key goal for memory disaggregation is to share memory across various workloads for better resource utilization and lower total cost of operation (TCO). However, pointer-traversal workloads across different users or applications can have different computation intensities (\ie, value of $\eta$), resulting in a complex performance and resource isolation problem at the memory nodes. Specifically, how should one assign an accelerator's logic and memory access across different pointer traversal workloads with varying values of $\eta$? We believe \name accelerator's scheduler (\S\ref{ssec:scheduler}) can be extended to support preemptions, enabling scheduling policies that limit the resources used by any particular user. Moreover, in order to extend this approach to distributed traversals (\S\ref{sec:distributed}), the accelerator could embed usage information within response packets so that either the programmable switch, other accelerators, or the compute node can decide when and how to limit a particular user's resource use across the entire cluster.

